Sampling-based Estimation of the Number of Distinct Values in Distributed Environment

In data mining, estimating the number of distinct values (NDV) is a fundamental problem with various applications. Existing methods for estimating NDV can be broadly classified into two categories: i) scanning-based methods, which scan the entire data and maintain a sketch to approximate NDV; and ii) sampling-based methods, which estimate NDV using sampling data rather than accessing the entire data warehouse. Scanning-based methods achieve a lower approximation error at the cost of higher I/O and more time. Sampling-based estimation is preferable in applications with a large data volume and a permissible error restriction due to its higher scalability. However, while the sampling-based method is more effective on a single machine, it is less practical in a distributed environment with massive data volumes. For obtaining the final NDV estimators, the entire sample must be transferred throughout the distributed system, incurring a prohibitive communication cost when the sample rate is significant. This paper proposes a novel sketch-based distributed method that achieves sub-linear communication costs for distributed sampling-based NDV estimation under mild assumptions. Our method leverages a sketch-based algorithm to estimate the sample's {\em frequency of frequency} in the {\em distributed streaming model}, which is compatible with most classical sampling-based NDV estimators. Additionally, we provide theoretical evidence for our method's ability to minimize communication costs in the worst-case scenario. Extensive experiments show that our method saves orders of magnitude in communication costs compared to existing sampling- and sketch-based methods.

==> rela.tex <==
\vspace{+1em}
\section{Other Related Works}
%{\hz {HZ: Maybe more intuitive descriptions instead of mathematical formulas. }}
\vspace{+0.5em}
\subsection{Other Related Sketch}
\header{\bf $\ell_p$ norms estimation. }Considering the norms of frequency, $\ell_0$ represent the distinct values of data. $\ell_p$ norms estimation is also a widely studied problem in stream models. Equation~\eqref{eq:fan} gives the relationship between $\ell_p$-norms with {\em frequency of frequency}. We just use $\ell_2$ norms of $f$ to estimate $\hat{D}_{CL1}$. If the estimators become more complicated than $\hat{D}_{CL1}$, we may use others $\ell_p$-norms to approximate. In other words, it is possible to derive an estimator by $\ell_p$ Sketch. $\ell_p$ sketch gives an estimation of the $\ell_p$ norm of vector $v$ in the communication complexity model. $\ell_p$ sketch utilizes a stable distribution proposed by Chambers et al.~\cite{chambers1976method} to estimate $\ell_p$ norms with a relative error. Limited by the updating time of the original $\ell_p$ sketch, Li~\cite{li2007very} proposes a faster updating method with a sparse random projection. 

\vspace{+0.5em}
\subsection{Other Estimates }
In this section, we will give some detail for complicated estimators. We also give the reason why our frameworks can handle different estimators. 

\header{\bf Chao Lee's Estimator. }
We have introduced the final expression of the first Chao Lee's Estimator before. In this part, we will give more details of Chao Lee's estimators.

We begin with some definitions of statistics. Sample coverage C is defined as the fraction of classes in the population that appears in the sample:
\begin{align*}
C=\sum_{j:n_j>0} \frac{N_j}{N}. 
\end{align*}
According to Turing et al.~\cite{good1953population}, $\hat{C}=1-f_1/n$ is used for sample coverage. To deal with the skew in the data, Chao and Lee~\cite{chao1992estimating} combine this coverage estimator with a correction term and obtain the estimator
\begin{equation}\label{eq:cl}
\hat{D}_{CL}=\frac{d}{\hat{C}}+\frac{n(1-\hat{C})}{\hat{C}}\hat{\gamma}^2,
\end{equation}
where $\hat{\gamma}^2$ is an estimator of $\gamma^2$, the squared coefficient of variation of the frequencies as follow.
\begin{align*}
\gamma^2=\frac{(1/D)\sum_{j=1}^D (N_j-\bar{N})^2 }{\bar{N}^2}. 
\end{align*}
According to~\cite{chao1992estimating}, there are following estimator of $\gamma^2$:
\begin{align*}
\hat{\gamma^2}=\max\left\{  \frac{\hat{D}_1 \sum i(i-1) f_i}{n^2-n-1},0 \right\},
\end{align*}
where $\hat{D}_1$ is an initial estimator $\hat{D}_1=d/\hat{C}$. From the above estimator of $\gamma^2$ and~\eqref{eq:cl},~\cite{chao1992estimating} constructs the following estimators:
\begin{equation}\label{eq:cl1}
\hat{D}_{CL1}=\frac{d}{\hat{C}}+\frac{n(1-\hat{C})}{\hat{C}}\hat{\gamma^2}.
\end{equation}
Chao and Lee~\cite{chao1992estimating} also introduce some improved estimators based on Equation~\eqref{eq:cl} and other assumptions, but for these Chao Lee's estimators, $\|f\|_2$ is enough to estimate.

\header{\bf Jackknife Estimator. }Haas et al.~\cite{haas1998estimating} propose a family of estimators, with the generalized jackknife approach~\cite{gray1972generalized}. It is of the form
\begin{equation}\label{eq:JE}
\hat{D}=d+K\frac{f_1}{n}.
\end{equation}
Different approximations for $K$ results in other estimators for $D$. At first, ~\cite{haas1998estimating} obtain the first-order estimator:
\begin{equation}\label{eq:uj1}
\hat{D}_{uj1}=\left( 1-\frac{(1-q)f_1}{n}  \right)^{-1} d. 
\end{equation}

The second-order estimator $\hat{D}_{uj2}$ is derived with the approximation of $\gamma^2$. Following but different form Chao and Lee~\cite{chao1992estimating},~\cite{haas1998estimating} uses a natural method-of-moments estimator $\hat{\gamma}^2_{Hass}(D)$ of $\gamma^2$ as follows.

\begin{equation}
\hat{\gamma}^2_{Haas}(\hat{D})=\max\left(0,\frac{\hat{D}}{n^2}\sum_{i=1}^n i(i-1)f_i +\frac{\hat{D}}{N}-1 \right). \label{eq:hass}
\end{equation}
With Taylor approximations for $K$ and~\eqref{eq:hass},~\cite{haas1998estimating} obtain the second-order jackknife estimator,
\begin{equation}\label{eq:uj2}
\hat{D}_{uj2}=\left( 1-\frac{(1-q)f_1}{n}  \right)^{-1} \left(d-\frac{f_1(1-q)\ln(1-q) \hat{\gamma}^2(\hat{D}_{uj1}) }{q} \right). 
\end{equation}
By replacing the expression $f_1/n$ with approximation to $E[f_1]/n$,~\cite{haas1998estimating} obtain a smoothed second-order jackknife estimator
\begin{equation}\label{eq:sj2}
\hat{D}_{sj2}=(1-(1-q)^{\tilde{N}})^{-1}(d-(1-q)^{\tilde{N}}\ln(1-q)N\hat{\gamma^2}(\hat{D}_{uj1}),
\end{equation}
where $\tilde{N}$ is an estimate of the average class size and is set to $N/\hat{D}_{uj1}$

Although Jackknife estimator is very complicated, $\|f\|_2$ will still be enough to estimate. Since $\hat{D}$ has a more concise form, we no longer put Jackknife estimator in the experimental comparison. 

\header{\bf Shlosser's Estimator. }Shlosser's estimator also conforms to the model~\eqref{eq:JE} with parameter
\begin{align*}
K=K_{Sh}= n \frac{f_1\sum_i (1-q)^i f_i }{ \sum_i iq(1-q)^{i-1} f_i }. 
\end{align*}
Replacing $K_{Sh}$ with approximation form,~\cite{haas1998estimating} obtain the following two estimators:
\begin{equation}\label{eq:sh2}
\hat{D}_{Sh2}=d+f_1\left(\frac{q(1+q)^{\tilde{N}-1}}{(1+q)^{\tilde{N}}-1}\right)\left( \frac{ \sum_{i=1}^n (1-q)^i f_i }{\sum_{i=1}^n iq(1-q)^{i-1}f_i}\right),
\end{equation}
where $\tilde{N}$ is an estimate of the average class size and is set to $N/\hat{D}_{uj1}$
%\begin{equation}\label{eq:sh3}
%\hat{D}_{Sh3}=d+f_1\left(\frac{\sum_{i=1}^n iq^2(1-q^2)^{i-1}f_i}{\sum_{i=1}^n(1-q)^i((1+q)^i-1)f_i}\right) \left(\frac{\sum_{i=1}^n(1-q)^if_i}{\sum_{i=1}^n iq(1-q)^{i-1}f_i}\right). 
%\end{equation}

When calculating $\hat{D}_{Sh2}$ for large $N$, it will result in floating point errors. Following~\cite{deolalikar2016extensive}, we can use $q/(1+q)$ to approximate the term in the first parentheses in~\eqref{eq:sh2}. For more complicated Shlosser's estimators, we still can resample to approximate, which also proves the applicability of our algorithm.

%For example, if we fix the resample ratio as $q^2$, we can solve the item $\sum_{i=1}^{n} i(1-q^2)^{i-1}f_i$.
